Online Label Aggregation: A Variational Bayesian Approach

Noisy labeled data is more a norm than a rarity for crowd sourced contents. It is effective to distill noise and infer correct labels through aggregation results from crowd workers. To ensure the time relevance and overcome slow responses of workers, online label aggregation is increasingly requested, calling for solutions that can incrementally infer true label distribution via subsets of data items. In this paper, we propose a novel online label aggregation framework, BiLA, which employs variational Bayesian inference method and designs a novel stochastic optimization scheme for incremental training. BiLA is flexible to accommodate any generating distribution of labels by the exact computation of its posterior distribution. We also derive the convergence bound of the proposed optimizer. We compare BiLA with the state of the art based on minimax entropy, neural networks and expectation maximization algorithms, on synthetic and real-world data sets. Our evaluation results on various online scenarios show that BiLA can effectively infer the true labels, with an error rate reduction of at least 10 to 1.5 percent points for synthetic and real-world datasets, respectively.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> samples/methods.tex <==
\subsection{Problem Definition}

We consider the online learning scenario shown in Figure~\ref{}. Data stream into the label aggregation model at different times in small sets $\bm{D}$ for training and aggregating. Each data instance $\bm{l}_i = \{l_{i0},...,l_{iK}\}$ contains redundant noisy labels of sample $i$. These noisy labels are provided by $K$ workers. $l_{ik} \in \bm{C}$ denotes the label of item $i$ given by worker $k \in \{1,...,K\}$, where $\bm{C} = \{1,...,C\}$ is the set of the possible classes. Not every worker might label all samples. If sample $i$ is not labeled by worker $k$, then the value of $l_{ik}$ is $-1$. We use $y_i \in \bm{C}$ to represent the unknown true label of a sample. In our online learning setting, our task is to continuously infer the values of $\{y_i| i \in \bm{D} \}$ for the current small set $\bm{D}$ in real time before receiving the next small set.


In order to define our optimization goal, we need some additional notations. We use $N$ to represent the total number of samples% during the full aggregating process which means the range of
, i.e. $i \in \{1,...,N\}$. $\bm{L} = \{\bm{l}_{1}, ..., \bm{l}_{N}\}$ is the collection of all observed noisy labels and $\bm{Y} = \{y_1,...,y_N\}$ is the collection of all unknown true labels.
\br{Is N the number of samples per small set or the total number of samples? I guess the total}

\subsection{The Label Aggregation Algorithm (\alg)}

In this section, we introduce our label aggregation algorithm (\alg) and define our optimization goal. \br{Add high level description (1-2) phrases of what the algorithm aims to do.}
The optimization goal is defined based on the principle of variational inference. The algorithm includes two components: a neural network $q$ and a generative model $p$. From the perspective of variational Bayesian inference, $q$ is an approximate distribution. The choice of $q$ and $p$ is very flexible. $q$ can be a multilayer perceptron (MLP), a convolutional neural network (CNN), or any other neural network. $p$ is the model to define how to generate the observed noisy labels $\bm{L}$ \br{do we generate all samples or only for the samples we have not yet received?}. Since we use a neural network as the approximate distribution to learn the label aggregation model, we need stochastic optimization to train the model parameters in $p$ and $q$. In order to apply stochastic optimization, the loss function should\br{must?} be differentiable respect to the model parameters in $p$. This is the only constraint of the definition of $p$. Besides, the close form of the posterior of model $p$ is needless. \br{Add why needless}. The relationship between $q$, $p$ and the loss function in \alg is shown in Figure~\ref{alg_loss}.

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.32]{samples/figures/alg_loss_function.pdf}
\end{center}
\caption{The relationship between $q$, $p$ and the loss function.\br{Add instance symbol ($\bm{l}$)}}
\label{alg_loss}
\end{figure}

\subsubsection{Definition of $p$ and $q$}
\br{sometime $\bm{l}$ and sometimes $\bm{l}_i$. do we need to be more consistent? Or add a note we drop subscript for, e.g., clarity?}
\br{I have the feeling that p is overloaded}
\br{I use $\hat{y}$ fro the predicted label} 

At first, we introduce the neural network $q$. Given an instance $\bm{l}_i$ of noisy redundant labels, we use $q$ to predict the corresponding unknown true label $\hat{y}_i$. $q$ is represented as a probability distribution $q_{\bm{\alpha}}(y=c|\bm{l})$, where
%$\bm{l}$ is the vector of collected redundant noisy labels for the sample and $\bm{\alpha}$
denotes the neural network parameters. % (e.g., weights, biases, etc. \br{do we need etc? what are we missing?}).
The output of the network is a C-dimensional vector $[q_{\bm{\alpha}}(y=c|\bm{l})]_{c=1}^{C}$, where the c-th element $q_{\bm{\alpha}}(y=c|\bm{l})$ is the probability that the true label of the input instance is class $c$. \br{The predicted label is given by the element with the highest probability.}

The set of noisy labels $\bm{L} = \{\bm{l}_1,...,\bm{l}_N\}$ only contains the observed instances $\bm{l}_i$. The corresponding true labels $y_i$ are unknown. The label aggregation task in this paper is to predict these unknown true labels according to $\bm{L}$. So it is an unsupervised learning task. In order to train $q$ we need an optimization goal. %Therefore, w
We define a generative model $p$ to describe the generative process behind the observed noisy data $\bm{L}$. Then we can define a loss function to guide the training according to some variational inference rules \cite{bishop2006pattern,wainwright2008graphical}. $p$ assumes that an instance $\bm{l}$ is generated from some conditional distributions $p_{\bm{\beta}}(\bm{l}|y)$, where $y$ denotes the unknown true label and $\bm{\beta}$ the model parameters of $p$. It also assumes that the true label $y$ is generated from a prior distribution $p_{\bm{\beta}}(y)$. The generative model $p$ potentially defines a posterior distribution:
\begin{equation}
p_{\bm{\beta}}(y|\bm{l}) = \frac{p_{\bm{\beta}}(\bm{l}|y)p_{\bm{\beta}}(y)}{p_{\bm{\beta}}(\bm{l})}.
\label{eq:gpos}
\end{equation}
We do not make many simplifying assumptions about $p$ except that the loss function should be differentiable with respect to $\bm{\beta}$.

\subsubsection{Optimization Goal}

Since we only have the observed noisy labels $\bm{L}$ in this learning task, maximizing the data likelihood of $\bm{L}$ is a reasonable optimization goal. We maximize the log data likelihood $\log p_{\bm{\beta}}(\bm{L})$ according to the evidence lower bound $\log p_{\bm{\beta}}(\bm{L}) = KL(q_{\bm{\alpha}}(\bm{Y}|\bm{L})||p_{\bm{\beta}}(\bm{Y}|\bm{L})) + L(q) \ge L(q)$, where $KL(\cdot)$ means the Kullback-Leibler divergence and $L(q) = \mathbbm{E}_{q_{\bm{\alpha}}(y_i|\bm{l}_i)}\left[ \log \frac{p_{\bm{\beta}}(\bm{L}, \bm{Y})}{q_{\bm{\beta}}(\bm{Y})} \right]$. We can see that we can maximize the lower bound of $\log p_{\bm{\beta}}(\bm{L})$ as we minimize $KL(q_{\bm{\alpha}}(\bm{Y}|\bm{L})||p_{\bm{\beta}}(\bm{Y}|\bm{L}))$. So, what we need to do is to find the consensus between the predictions of $q$ and $p$. We apply $KL(q_{\bm{\alpha}}(\bm{Y}|\bm{L})||p_{\bm{\beta}}(\bm{Y}|\bm{L}))$ as our loss function. We minimize it during the training process.

We assume that each collected label is independently generated. The instances in $\bm{L}$ are independent with each other. Plugging $q_{\bm{\alpha}}(\bm{Y}|\bm{L}) = \prod_i q_{\bm{\alpha}}(y_i|\bm{l}_i)$ and $p_{\bm{\beta}}(\bm{Y}|\bm{L}) = \prod_i p_{\bm{\beta}}(y_i|\bm{l}_i)$ into the loss function, we have:
\begin{align}
KL(q_{\bm{\alpha}} & (\bm{Y}|\bm{L})||p_{\bm{\beta}}(\bm{Y}|\bm{L})) 
    = \sum_{i=1}^{N} -\mathbbm{E}_{q_{\bm{\alpha}}(y_i|\bm{l}_i)}\left[ \log \frac{p_{\bm{\beta}}(y_i|\bm{l}_i)}{q_{\bm{\alpha}}(y_i|\bm{l}_i)} \right] \notag \\
    &= \sum_{i=1}^{N} KL(q_{\bm{\alpha}}(y_i|\bm{l}_i)||p_{\bm{\beta}}(y_i|\bm{l}_i))
    \label{kl_sum}
\end{align}
Equation (\ref{kl_sum}) cannot be directly used to train $q$ and $p$, because the expression of $p_{\bm{\beta}}(y|\bm{l})$ is unknown. The exact expression of the posterior $p_{\bm{\beta}}(y|\bm{l})$ may be intractable. So we have to further rewrite the loss function. According to (\ref{eq:gpos}), we have
\begin{align}
&KL(q_{\bm{\alpha}} (y|\bm{l})||p_{\bm{\beta}}(y|\bm{l})) 
    = -\mathbbm{E}_{q_{\bm{\alpha}}(y|\bm{l})}\left[ \log \frac{p_{\bm{\beta}}(y|\bm{l})}{q_{\bm{\alpha}}(y|\bm{l})} \right] \notag \\
    &= -\mathbbm{E}_{q_{\bm{\alpha}}(y|\bm{l})}\left[ \log \frac{p_{\bm{\beta}}(y)}{q_{\bm{\alpha}}(y|\bm{l})} + \log p_{\bm{\beta}}(\bm{l}|y) \right] + const \notag \\
    &= KL(q_{\bm{\alpha}}(y|\bm{l})||p_{\bm{\beta}}(y)) - \mathbbm{E}_{q_{\bm{\alpha}}(y|\bm{l})}\left[ \log p_{\bm{\beta}}(\bm{l}|y) \right] + const
    \label{kl_calc}
\end{align}
To simplify the notations, we use $\theta = \{\bm{\alpha}, \bm{\beta}\}$ to represent the total model parameter in our algorithm. According to (\ref{kl_sum}) and (\ref{kl_calc}) the loss function is rewritten as
\begin{align}
\mathcal{F}(\theta ; \bm{L}) =& \frac{1}{N}\sum_{i=1}^{N} \{ KL(q_{\bm{\alpha}}(y_i|\bm{l}_i)||p_{\bm{\beta}}(y_i)) - \mathbbm{E}_{q_{\bm{\alpha}}(y_i|\bm{l}_i)}\left[ \log p_{\bm{\beta}}(\bm{l}_i|y_i) \right] \}
\label{eq:lossf}
\end{align}
where the constant is ignored and the loss function is rescaled by $1/N$. This will not affect the optimization result.

\subsubsection{Training}

We are going to solve the following optimization problem
\begin{equation*}
\hat{\theta} = \mathop{\arg\min}_{\theta} \mathcal{F}(\theta; \bm{L}).
\end{equation*}
during the training. The optimization problem is solved by stochastic first-order optimization. The update rule of the model parameter is shown in Algorithm~\ref{nn-mc}. As what we discussed in Section~\ref{system_scenarios}, in order to continuously aggregate small sets of noisy labels, we have to apply mini-batch training to update the parameter $\theta$. So the loss function that we use for training is
\begin{align}
&f(\theta;\bm{L}^{(M)}) = \notag\\
&\frac{1}{M}\sum_{i=1}^{M} \left\{ KL(q_{\bm{\alpha}}(y_i|\bm{l}_i)||p_{\bm{\beta}}(y_i)) - \mathbbm{E}_{q_{\bm{\alpha}}(y_i|\bm{l}_i)}\left[ \log p_{\bm{\beta}}(\bm{l}_i|y_i) \right] \right\},
\label{eq:miniloss}
\end{align}
where $\bm{L}^{(M)}$ is a mini-batch sampled from $\bm{L}$, and $M$ denotes the minibatch size. The gradient of $f(\theta; \bm{L}^{(M)})$ is required to update the model parameters. Before calculating the gradient, we need to define the expression of the KL divergence and the expectation term. The unobserved variables $y_i$ are discrete variables that take values from $1$ to $C$. Therefore, we have the following expressions
\begin{equation}
KL(q_{\bm{\alpha}}(y|\bm{l})||p_{\bm{\beta}}(y)) = -\sum_{c=1}^{C}q_{\bm{\alpha}}(c|\bm{l})\log \frac{p_{\bm{\beta}}(c)}{q_{\bm{\alpha}}(c|\bm{l})},
\label{eq:klcalc}
\end{equation}
\begin{equation}
\mathbbm{E}_{q_{\bm{\alpha}}(y|\bm{l})}\left[ \log p_{\bm{\beta}}(\bm{l}|y) \right] = \sum_{c=1}^{C}q_{\bm{\alpha}}(c|\bm{l})\log p_{\bm{\beta}}(\bm{l}|c),
\label{eq:ecalc}
\end{equation}
where $q_{\bm{\alpha}}(c|\bm{l})$ is the c-th element of the neural network output. We can see that we don't have to apply any approximate approach for calculating the expectation terms in our loss function, so we don't have the problem of the high variance of the loss function which is mentioned in stochastic Bayesian inference \cite{paisley2012variational}.
According to (\ref{eq:klcalc}) and (\ref{eq:ecalc}), the values of $f(\theta;\bm{L}^{(M)})$ and the corresponding stochastic gradient $\nabla_{\theta} f(\theta;\bm{L}^{(M)})$ can be easily computed. Now, we have defined all necessary things in the framework for constructing online label aggregation models.



\subsection{The Label Aggregation Model}

\subsubsection{Definition}
In this section, we will introduce an online label aggregation model, \model, which is based on the aforementioned algorithm framework. This model can be applied to aggregate discrete noisy labels. In order to define the model and get the exact form of the loss function $f$, we need to decide the concrete form of $q$ and $p$. At first we define the form of the approximate distribution $q$. In \model, $q$ is a fully connected neural network with a softmax activation function on the last layer. It inputs an instance $\bm{l}$ and outputs a distribution $q_{\bm{\alpha}}(y|\bm{l})$, where $\bm{\alpha}$ denotes the network parameters (e.g., weights and biases). 

Next we design a generative model $p$ for \model to define the generation of the observed noisy labels $\bm{l}$. As shown in (\ref{eq:klcalc}) and (\ref{eq:ecalc}), in order to compute the loss function and its gradient, we need to define the expressions of $p_{\bm{\beta}}(\bm{l}|y)$ and $p_{\bm{\beta}}(y)$. Since every element in an instance is independently collected from different workers, in this model p, we assume that the $k$-th element in an instance is generated by a independent distribution $\bm{\psi}_{ck}$ when the true label of the sample is $c$. This distribution is defined as
\begin{equation}
\bm{\psi}_{ck} = softmax(\bm{\omega}_{ck}),
\label{eq:psi}
\end{equation}
where $\bm{\omega}_{ck}$ is a C-dimensional vector. Then $p_{\bm{\beta}}(\bm{l}|y = c)$ can be defined as
\begin{equation}
p_{\bm{\beta}}(\bm{l}_i|y_i = c) = \prod_{k \in \bm{S}_i}\psi_{ck,l_{ik}}, c \in [C],
\end{equation}
where $\psi_{ck,l_{ik}}$ is the $l_{ik}$-th element of $\bm{\psi}_{ck}$. Since the softmax function is derivable, $\bm{\omega}_{ck}$ can be updated by stochastic optimization. In this model, the prior distribution $p_{\bm{\beta}}(y)$ is a multinomial distribution and is estimated by
\begin{equation}
    \hat{p}_{\bm{\beta}}(y=c) = \frac{\sum_{i}\sum_{k}\mathbbm{I}(l_{ik}=c)}{\sum_{i}\sum_{k}\mathbbm{I}(l_{ik} \neq -1)}, c \in [C],
\label{eq:priorest}
\end{equation}
where the values of the estimators can be calculated by the result of counting the observed labels. Since $p_{\bm{\beta}}(y)$ is fixed, we introduce a hyperparameter $\zeta$ to constrain the Kullback-Leibler divergence term in the loss function (\ref{eq:miniloss}). We regard this constrained term as a regularizer. Then, using (\ref{eq:klcalc}) and (\ref{eq:ecalc}) the mini-batch loss function used in practice is
\begin{align}
f(\theta;\bm{L}^{(M)}) =& 
             -\frac{1}{M}\sum_{i=1}^{M} \Big\{ \zeta \sum_{c=1}^{C}q_{\bm{\alpha}}(c|\bm{l}_i)\log \frac{p_{\bm{\beta}}(c)}{q_{\bm{\alpha}}(c|\bm{l}_i)} \notag \\ &+ \sum_{c=1}^{C}q_{\bm{\alpha}}(c|\bm{l}_i)\log p_{\bm{\beta}}(\bm{l}_i|c) \Big\},
\label{eq:minilossprac}
\end{align}


Then let's discuss the full procedure of the model. The details of the completed online label aggregation model \model is illustrated in Algorithm~$1$. \model will continuously receive new noisy labels set $\bm{L}^{(s)}$ which contains multiple redundant noisy label instances. The size of each set could be different. At the beginning, we will accumulate few sets of noisy labels to construct a initial set $\bm{L^{*}}$. This initial set will be applied to initialize the model parameter $\bm{\beta} = \{\bm{\omega}_{ck}\}$ and the prior estimator $\hat{p}_{\bm{\beta}}(y)$, where $\bm{\beta}$ can be initialized by its definition and majority voting. We will aggregate the initial set and obtain the corresponding predicted true labels. After the initialization, we can start the online aggregating. For each arriving set $\bm{L}^{(s)}$, we use it to update the model parameter $\theta$ and then aggregate it using the updated $\theta$. The update and aggregating process of \model is illustrated in the function UpdateAndAggregate. The loss function $f$ that we use in the update process is shown in Eq(\ref{eq:minilossprac}).

\begin{algorithm}
\caption{The Online Label Aggregation Model \model. The model parameters are represented by $\theta = \{\bm{\alpha}, \bm{\beta}\}$, where $\bm{\alpha}=\{\bm{W}_1,\bm{W}_2,\bm{b}_1,\bm{b}_2\}$ and $\bm{\beta} = \{\bm{\omega}_{ck}\}$.}
\label{alg_bila}
\DontPrintSemicolon
  \textbf{Set:} learning rate $\mu > 0, exponential decay rate \gamma \in [0, 1), \epsilon = 10^{-8}, t = 1$ \\
  \textbf{Input:} Continuously receive new noisy labels set $\bm{L}^{(s)} = \{\bm{l}\}$ \\
  Accumulate few sets to construct the initial set $\bm{L^{*}}$ \\
  Initialize $\theta$ using $\bm{L^{*}}$ \\
  $\bm{Y^{*}} = $ UpdateAndAggregate($\bm{L^{*}}$) \\
  \textbf{Output:} The aggregated labels $\bm{Y^{*}}$ \\
  \For{each arriving set $\bm{L}^{(s)}$}    
    { 
        $\bm{Y}^{(s)} = $ UpdateAndAggregate($\bm{L}^{(s)}$) \\
        \textbf{Output:} The aggregated labels $\bm{Y}^{(s)}$
    }
 
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FUpdateAndAggregate{$\bm{L}^{(s)}$}}{
        \For{number of training epochs}
        {
            \For{number of minibatchs}
            {
                Sample a batch $\bm{L}^{(M)}=\{\bm{l}_1,...,\bm{l}_M \}$ from $\bm{L}^{(s)}$ \\
                \tcc{Calculate each term in $f$, Eq(\ref{eq:minilossprac})}
                \For{$c = 1,...,C$}
                {
                    \For{$k = 1,...,K$}
                    {
                        $\bm{\psi}_{ck} = softmax(\bm{\omega}_{ck})$
                    }
                }
                \For{instance $i = 1,...,M$}
                {
                    $\bm{h} = \bm{W}_2~tanh(\bm{W}_1\bm{l}_i + \bm{b}_1)+\bm{b}_2$ \\
                    $[q_{\bm{\alpha}}(t=c|\bm{l}_i)]_{c=1}^{C} = softmax(\bm{h})$ \\
                    \For{$c = 1,...,C$}
                    {
                        $\log g_{\bm{\beta}}(\bm{l}_i|t = c) = \sum_{k \in \bm{S}_i}\log \psi_{ck,l_{ik}}$
                    }
                }
                \tcc{update the model parameters $\theta$}
                $g_t \leftarrow \bigtriangledown_{\theta} f_t(\theta_t)$ \\
                $v_t \leftarrow \gamma \cdot v_{t-1} + (1-\gamma) \cdot (g_t \odot g_t)$ \\
                $\mu_t = (\mu / \sqrt{t}) \cdot \sqrt{1-\gamma^{t}}$ \\
                $\theta_{t+1} \leftarrow \theta_t - \mu_t \cdot g_t/(\sqrt{v_t} + \epsilon)$ \\
                $t \leftarrow t+1$ \tcp*{count the time step}
            }
        }
        Get new confusion matrices $\bm{\pi}$ by the updated $\bm{\beta}$ \\
        Infer the aggregated labels $\bm{Y}^{(s)}$ by $\bm{\pi}$ \\
        \KwRet $\bm{Y}^{(s)}$
  }
\end{algorithm}

\subsubsection{Inferring the aggregated labels}
Before introducing how to infer the aggregated label $y$ (the predicted true label) for each sample $\bm{l}$, we would like to discuss the connection between the generative model $p$ of \model and confusion matrix which is a well known concept in label aggregation field. A confusion matrix $\bm{\pi}_{c,z}^{(k)}$ of worker $k$ is a matrix for describing the worker's labeling behavior \cite{dawid1979maximum}. It's element $\pi_{c,z}^{(k)} = p(l_{ik} = z | y_i =c)$ is the probability that worker $k$ assigns $z$ to the sample when the true label is $c$. According to the definition of $p$, we have $\psi_{ck,z} = p_{\bm{\beta}}(l_{ik} = z| y_i=c)$ which is corresponding to $\pi_{c,z}^{(k)}$. Therefore, in actually, we can easily construct the confusion matrices of the workers after learning the parameters $\bm{\beta}=\{\bm{\omega_{ck}}\}$. Then, the inferring problem becomes trivial. After obtaining the values of the confusion matrices, we can infer the aggregated label of a sample by maximizing the data likelihood of the observed noisy labels.

